Engineering faster double-array Aho-Corasick automata

Multiple pattern matching in strings is a fundamental problem in text processing applications such as regular expressions or tokenization. This paper studies efficient implementations of double-array Aho-Corasick automata (DAACs), data structures for quickly performing the multiple pattern matching. The practical performance of DAACs is improved by carefully designing the data structure, and many implementation techniques have been proposed thus far. A problem in DAACs is that their ideas are not aggregated. Since comprehensive descriptions and experimental analyses are unavailable, engineers face difficulties in implementing an efficient DAAC. In this paper, we review implementation techniques for DAACs and provide a comprehensive description of them. We also propose several new techniques for further improvement. We conduct exhaustive experiments through real-world datasets and reveal the best combination of techniques to achieve a higher performance in DAACs. The best combination is different from those used in the most popular libraries of DAACs, which demonstrates that their performance can be further enhanced. On the basis of our experimental analysis, we developed a new Rust library for fast multiple pattern matching using DAACs, named Daachorse, as open-source software at https://github.com/daac-tools/daachorse. Experiments demonstrate that Daachorse outperforms other AC-automaton implementations, indicating its suitability as a fast alternative for multiple pattern matching in many applications.

==> only-figures.tex <==
\begin{figure}[tb]
\centering
\subfloat[AC automaton]{
\includegraphics[scale=0.8]{figs/examples/ac.pdf}
\label{fig:ac:pma}
}
\subfloat[Trie]{
\includegraphics[scale=0.8]{figs/examples/trie.pdf}
\label{fig:ac:trie}
}
\caption{
Examples of (a) an AC automaton for the dictionary of Table 1 and (b) its trie part.
Transitions are depicted by solid line arrows.
$\delta(0,\Str{b}) = 2$, $\delta(2,\Str{a}) = 5$, and $\delta(2,\Str{c}) = -1$.
We depict the mappings of the failure function (except ones to the initial state) by dotted line arrows.
$f(4)=2$, $f(5)=1$, $f(6)=2$, $f(7)=3$, $f(8)=4$, and $f(s) = 0$ for the other states $s$.
Output states are shaded and associated with pattern indices (drawn from $\Str{A},\Str{B},\Str{C},\dots$).
$h(2)=\{\Str{B}\}$, $h(4)=\{\Str{A,B}\}$, $h(6)=\{\Str{E,B}\}$, $h(7)=\{\Str{F}\}$, $h(8)=\{\Str{C,A,B}\}$, $h(9)=\{\Str{D}\}$, and $h(s) = \emptyset$ for the other states $s$.
}
\label{fig:ac}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[scale=0.85]{figs/examples/datrie.pdf}
\caption{
\Name{BASE} and \Name{CHECK} implementing the transition function $\delta$ of Figure \ref{fig:ac:trie}.
$\Sigma = \{ \Str{a} = 0,\Str{b} = 1,\Str{c} = 2,\Str{d} = 3 \}$.
The state ids are assigned to satisfy Equation (2).
$\delta(0,\Str{b}) = 2$ is simulated by $\Name{BASE}[0] + \Str{b} = 2$ and $\Name{CHECK}[2] = 0$.
$\delta(2,\Str{d}) = -1$ is simulated by $\Name{BASE}[2] + \Str{d} = 8$ and $\Name{CHECK}[8] \neq 2$.
The state id 7 is a vacant id because its element does not represent any state of the original trie.
}
\label{fig:da:trie}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[scale=0.85]{figs/examples/daac_1.pdf}
\caption{
DAAC for the AC automaton in Figure \ref{fig:ac:pma}.
}
\label{fig:da}
\end{figure}

\begin{figure}[tb]
\centering
\subfloat[\Name{Shared}]{
\includegraphics[scale=0.9]{figs/examples/out-shared.pdf}
\label{fig:out:shared}
}\\
\subfloat[\Name{Forest}]{
\includegraphics[scale=0.9]{figs/examples/out-forest.pdf}
\label{fig:out:forest}
}
\caption{
Examples of approaches to store output sets of Figure \ref{fig:da}.
}
\label{fig:out}
\end{figure}

\begin{figure}[tb]
\centering
\subfloat[\Name{Individual}]{
\includegraphics[scale=0.9]{figs/examples/layout-indi.pdf}
\label{fig:layout:indi}
}\\
\subfloat[\Name{Packed}]{
\includegraphics[scale=0.9]{figs/examples/layout-pack.pdf}
\label{fig:layout:pack}
}
\caption{
Illustrations of memory layouts of arrays.
}
\label{fig:layout}
\end{figure}

\begin{figure}[tb]
\centering
\includegraphics[scale=0.9]{figs/examples/xorda.pdf}
\caption{
\Name{BASE} and \Name{CHECK} implementing the transition function $\delta$ of Figure \ref{fig:ac:trie} based on Equation (6).
The block size $B$ is four, since $|\Sigma| = 4$ and $B = 2^{\Ceil{\log_2 4}}$.
Destination states 5 and 7 from state 1 are placed in the same block, i.e., $\Floor{5/4} = \Floor{7/4} = 1$.
}
\label{fig:vacant:xor}
\end{figure}

\begin{figure}[tb]
\centering
\subfloat[\Name{SkipForward}]{
\includegraphics[scale=0.9]{figs/examples/skipT.pdf}
\label{fig:vacant:t}
}\\
\subfloat[\Name{SkipDense}]{
\includegraphics[scale=0.9]{figs/examples/skipS.pdf}
\label{fig:vacant:s}
}
\caption{
Illustrations of skipping techniques.
}
\label{fig:vacant}
\end{figure}

\begin{figure}[tbp]
\centering
\subfloat[\Name{BFS}]{
\includegraphics[scale=0.9]{figs/examples/BFS.pdf}
\label{fig:ex:order:lexbfs}
}\\
\subfloat[\Name{DFS}]{
\includegraphics[scale=0.9]{figs/examples/DFS.pdf}
\label{fig:ex:order:lexdfs}
}
\caption{
Examples of resultant \Name{BASE} and \Name{CHECK} arrays constructed with \Name{BFS} and \Name{DFS} for a dictionary of four patterns \Str{aa}, \Str{bbb}, \Str{cccc}, and \Str{ddddd}.
$\Sigma = \{ \Str{a} = 0,\Str{b} = 1,\Str{c} = 2,\Str{d} = 3 \}$.
The state ids are determined based on Equation (2).
In the construction, vacant searches are performed from the forward to use smaller state ids first.
A set of outgoing transition labels (or $E$) is scanned in the lexicographical order (i.e., the figures show the results of \Name{LexBFS} and \Name{LexDFS} more precisely).
In both cases, the initial state and its destination states have identical ids (i.e., states 0 to 4).
This is because the initial state id is always fixed to 0, and its destination state ids are fixed to $\Name{BASE}[0]$ to satisfy Equation (2).
The deeper states have different ids in accordance with the order of visiting states.
}
\label{fig:ex:order}
\end{figure}

\begin{figure}[btp]
\centering
\subfloat[Matching time (ms)]{
\label{fig:layout:match:time}
\includegraphics[scale=0.5]{figs/layout/enwords-match.pdf}
\includegraphics[scale=0.5]{figs/layout/jawords-match.pdf}
\includegraphics[scale=0.5]{figs/layout/jachars-match.pdf}
}\\
\subfloat[Number of L1-load misses occurring during a pattern matching]{
\label{fig:layout:match:l1-cache}
\includegraphics[scale=0.5]{figs/layout/enwords-l1_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jawords-l1_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jachars-l1_miss.pdf}
}\\
\subfloat[\R{Number of L3-load misses occurring during a pattern matching}]{
\label{fig:layout:match:l3-cache}
\includegraphics[scale=0.5]{figs/layout/enwords-l3_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jawords-l3_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jachars-l3_miss.pdf}
}
\caption{
Comparison results on matching time and cache efficiency for the \Name{Individual} and \Name{Packed} layouts.
}
\label{fig:layout:match}
\end{figure}

\begin{figure}[btp]
\centering
\subfloat[Number of CPU instructions occurring during a pattern matching]{
\label{fig:layout:other:instructions}
\includegraphics[scale=0.5]{figs/layout/enwords-instructions.pdf}
\includegraphics[scale=0.5]{figs/layout/jawords-instructions.pdf}
\includegraphics[scale=0.5]{figs/layout/jachars-instructions.pdf}
}\\
\subfloat[Number of branch misses occurring during a pattern matching]{
\label{fig:layout:other:branch_miss}
\includegraphics[scale=0.5]{figs/layout/enwords-branch_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jawords-branch_miss.pdf}
\includegraphics[scale=0.5]{figs/layout/jachars-branch_miss.pdf}
}
\caption{
\R{Comparison results on CPU instructions and branch misses for the \Name{Individual} and \Name{Packed} layouts.}
}
\label{fig:layout:other}
\end{figure}

\begin{figure}[btp]
\centering
\subfloat[The average number of verifications per vacant search]{
\label{fig:exp:constr:verif}
\includegraphics[scale=0.6]{figs/construction/verif-jawords-bytewise-compact.pdf}
\includegraphics[scale=0.6]{figs/construction/verif-jachars-charwise.pdf}
}\\
\subfloat[Construction time in seconds]{
\label{fig:exp:constr:time}
\includegraphics[scale=0.6]{figs/construction/time-jawords-bytewise-compact.pdf}
\includegraphics[scale=0.6]{figs/construction/time-jachars-charwise.pdf}
}
\caption{
Experimental results for verifications and construction times when using \Name{Chain}, \Name{SkipForward}, or \Name{SkipDense}.
}
\label{fig:exp:constr}
\end{figure}

\begin{figure}[btp]
\centering
\includegraphics[scale=0.5]{figs/order/enwords-bytewise.pdf}
\includegraphics[scale=0.5]{figs/order/jawords-bytewise.pdf}
\includegraphics[scale=0.5]{figs/order/jachars-bytewise.pdf}\\
\includegraphics[scale=0.5]{figs/order/enwords-charwise.pdf}
\includegraphics[scale=0.5]{figs/order/jawords-charwise.pdf}
\includegraphics[scale=0.5]{figs/order/jachars-charwise.pdf}
\caption{
Matching times in milliseconds for different traversal orders.
}
\label{fig:order}
\end{figure}

\begin{figure}[btp]
\centering
\includegraphics[scale=0.6]{figs/order/depth-counts.pdf}
\caption{
The number of visiting states at each depth during a pattern matching.
}
\label{fig:order:counts}
\end{figure}

\begin{figure}[tbp]
\centering
\subfloat[Matching time (ms)]{
\includegraphics[scale=0.5]{figs/comparison/enwords-match.pdf}
\includegraphics[scale=0.5]{figs/comparison/jawords-match.pdf}
\includegraphics[scale=0.5]{figs/comparison/jachars-match.pdf}
\label{fig:comparison:match}
}\\
\subfloat[Construction time (ms)]{
\includegraphics[scale=0.5]{figs/comparison/enwords-constr.pdf}
\includegraphics[scale=0.5]{figs/comparison/jawords-constr.pdf}
\includegraphics[scale=0.5]{figs/comparison/jachars-constr.pdf}
\label{fig:comparison:constr}
}\\
\subfloat[Memory usage (KiB)]{
\includegraphics[scale=0.5]{figs/comparison/enwords-size.pdf}
\includegraphics[scale=0.5]{figs/comparison/jawords-size.pdf}
\includegraphics[scale=0.5]{figs/comparison/jachars-size.pdf}
\label{fig:comparison:size}
}
\caption{
Comparison results with the Daachorse and Aho-corasick libraries.
(a) The matching time is plotted in a linear scale because the time complexity is not linear over the number of patterns.
(b) The construction time and (c) the memory usage are plotted in a logarithmic scale because the complexities are linear over the number of patterns.
}
\label{fig:comparison}
\end{figure}


==> only-tables.tex <==
\begin{table}[p]
\footnotesize
\centering
\caption{
A dictionary $\mathcal{D}$ of six patterns (used in examples throughout this paper).
Patterns are indexed with upper-case letters $\Str{A},\Str{B},\Str{C},\dots$ instead of numbers in the examples.
Elements in the integer alphabet $\Sigma$ are denoted with lower-case letters.
$\Sigma = \{ \Str{a} = 0,\Str{b} = 1,\Str{c} = 2,\Str{d} = 3 \}$.
}
\label{tab:dictioanry}
\begin{tabular}{|c||c|}
\hline
Index & Pattern \\
\hline\hline
\Str{A} & \Str{ab} \\
\Str{B} & \Str{b} \\
\Str{C} & \Str{bab} \\
\Str{D} & \Str{bac} \\
\Str{E} & \Str{db} \\
\Str{F} & \Str{dd} \\
\hline
\end{tabular}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
Summary of implementation techniques in DAACs.
``Selected'' indicates the techniques selected to be the best through our experiments in Section \ref{sect:exp} and are used in our Daachorse library.
}
\label{tab:summary}
\subfloat[Approaches to store output sets (Section \ref{sect:tech:out})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References  & Selected \\
\hline\hline
\Name{Simple} & Arranging pattern indices in a simple manner & Conventional & \\ \hline
\Name{Shared} & Merging some common parts of pattern indices in \Name{Simple} & This study & \\ \hline
\Name{Forest} & Storing pattern indices in a forest structure & \cite{belazzougui2010succinct} & \checkmark{} \\ \hline
\end{tabular}
}\\
\subfloat[Schemes to handle strings of multibyte characters (Section \ref{sect:tech:wise})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References & Selected \\
\hline\hline
\Name{Bytewise} & Slicing multibyte characters into byte sequences & Conventional & \checkmark{} \\ \hline
\Name{Charwise} & Handling multibyte characters as code points in Unicode & Conventional & \\ \hline
\Name{Mapped} & Mapping code points in the frequency order & \cite{liu2011compression,norimatsu2016fast} & \checkmark{} \\ \hline
\end{tabular}
}\\
\subfloat[Memory layouts of double-arrays (Section \ref{sect:tech:layout})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References & Selected \\
\hline\hline
\Name{Individual} & Maintaining arrays \Name{BASE}, \Name{CHECK}, \Name{FAIL}, and \Name{OUTPOS} individually & Conventional & \\ \hline
\Name{Packed} & Arranging values in the arrays cache-efficiently & e.g., \cite{morita2001fast,yata2007compact} & \checkmark{} \\ \hline
\end{tabular}
}\\
\subfloat[Formats of double-arrays in \Name{Bytewise} scheme (Section \ref{sect:tech:format})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References & Selected \\
\hline\hline
\Name{Basic} & Implementing \Name{BASE}, \Name{CHECK}, \Name{FAIL}, and \Name{OUTPOS} as arrays of four-byte integers & Conventional & \\ \hline
\Name{Compact} & Compressing \Name{CHECK} into a byte array  & \cite{yata2007compact} & \checkmark{} \\ \hline
\end{tabular}
}\\
\subfloat[Approaches to accelerate vacant searches (Section \ref{sect:tech:constr})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References & Selected \\
\hline\hline
\Name{Chain} & Visiting only vacant ids with a linked list & \cite{morita2001fast} & \\ \hline
\Name{SkipForward} & Searching for only the last $L$ blocks & \cite{morita2001fast,dartsclone} & \checkmark{} \\ \hline
\Name{SkipDense} & Searching for only blocks in which the vacant proportion is no less than $\tau$ & This study & \\ \hline
\end{tabular}
}\\
\subfloat[Traversal orders in construction (Section \ref{sect:tech:order})]{
\begin{tabular}{|c||l|c|c|}
\hline
Technique & Brief description & References & Selected \\
\hline\hline
\Name{LexBFS} & Visiting states with breadth-first search and transition labels in the lexicographical order & Conventional & \\ \hline
\Name{FreqBFS} & Visiting states with breadth-first search and transition labels in the frequency order & Conventional & \\ \hline
\Name{LexDFS} & Visiting states with depth-first search and transition labels in the lexicographical order & Conventional & \checkmark{} \\ \hline
\Name{FreqDFS} & Visiting states with depth-first search and transition labels in the frequency order & Conventional & \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{Basic statistics of dictionaries.}
\label{tab:dataset}
\subfloat[Average pattern length in bytes]{
\label{tab:dataset:lenbyte}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 5.0 & 6.6 & 7.1 & 7.5 \\
\Name{JaWord} & 5.7 & 6.7 & 8.7 & 14.5 \\
\Name{JaChars} & 4.9 & 6.3 & 7.3 & 8.0 \\
\hline
\end{tabular}
}
\subfloat[Average pattern length in characters]{
\label{tab:dataset:lenchar}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 5.0 & 6.6 & 7.1 & 7.5 \\
\Name{JaWord} & 1.9 & 2.3 & 3.0 & 5.2 \\
\Name{JaChars} & 1.8 & 2.3 & 2.7 & 2.9 \\
\hline
\end{tabular}
}
\subfloat[Alphabet size in the \Name{Bytewise} scheme]{
\label{tab:dataset:alphbyte}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 226 & 226 & 239 & 239 \\
\Name{JaWord} & 233 & 238 & 239 & 244 \\
\Name{JaChars} & 233 & 233 & 238 & 239 \\
\hline
\end{tabular}
}\\
\subfloat[Alphabet size in the \Name{Charwise} scheme]{
\label{tab:dataset:alphchar}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 8,226 & 9,632 & 63,289 & 65,532 \\
\Name{JaWord} & 39,640 & 57,345 & 64,017 & 1,048,766 \\
\Name{JaChars} & 39,640 & 40,845 & 57,345 & 64,017 \\
\hline
\end{tabular}
}
\subfloat[Mapped alphabet size in the \Name{Mapped} scheme]{
\label{tab:dataset:alphcharm}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 83 & 104 & 177 & 472 \\
\Name{JaWord} & 669 & 2,262 & 4,806 & 10,809 \\
\Name{JaChars} & 483 & 1,648 & 2,990 & 4,773 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{The number of occurrences in pattern matching per sentence.}
\label{tab:dataset:occur}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 47.2 & 93.4 & 126.2 & 150.8 \\
\Name{JaWord} & 25.8 & 38.0 & 46.7 & 49.0 \\
\Name{JaChars} & 36.6 & 54.6 & 69.7 & 79.9 \\
\hline
\end{tabular}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
Experimental results for approaches to store output sets: \Name{Simple}, \Name{Shared}, and \Name{Forest}.
For memory usage, the total of \Name{OUTPUT} and \Name{TERM} is reported in \Name{Simple} and \Name{Shared}, and the total of \Name{OUTPUT} and \Name{PARENT} is reported in \Name{Forest}.
The last two rows in Tables (a)--(c) show the different ratios for each result.
}
\label{tab:output}
\subfloat[Length of \Name{OUTPUT} ($\times 10^3$)]{
\label{tab:output:length}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Approach & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Simple} & 1.60 & 29.2 & 412 & 4,988 & 1.46 & 18.7 & 247 & 3,615 & 1.68 & 21.6 & 252 & 2,779 \\
\Name{Shared} & 1.46 & 26.2 & 362 & 4,377 & 1.31 & 16.7 & 218 & 3,132 & 1.40 & 17.7 & 217 & 2,497 \\
\Name{Forest} & 1.00 & 10.0 & 100 & 1,000 & 1.00 & 10.0 & 100 & 1,000 & 1.00 & 10.0 & 100 & 1,000 \\
\hline
\Name{Shared}/\Name{Simple} & 0.92 & 0.90 & 0.88 & 0.88 & 0.89 & 0.89 & 0.88 & 0.87 & 0.83 & 0.82 & 0.86 & 0.90 \\
\Name{Forest}/\Name{Simple} & 0.63 & 0.34 & 0.24 & 0.20 & 0.68 & 0.53 & 0.40 & 0.28 & 0.60 & 0.46 & 0.40 & 0.36 \\
\hline
\end{tabular}
}\\
\subfloat[Memory usage (KiB)]{
\label{tab:output:memory}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Approach & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Simple} & 12.5 & 228 & 3,219 & 38,968 & 11.4 & 146 & 1,932 & 28,244 & 13.1 & 168 & 1,971 & 21,707 \\
\Name{Shared} & 11.4 & 205 & 2,830 & 34,192 & 10.2 & 131 & 1,703 & 24,473 & 10.9 & 139 & 1,692 & 19,507 \\
\Name{Forest} & 11.7 & 117 & 1,172 & 11,719 & 11.7 & 117 & 1,172 & 11,719 & 11.7 & 117 & 1,172 & 11,719 \\
\hline
\Name{Shared}/\Name{Simple} & 0.92 & 0.90 & 0.88 & 0.88 & 0.89 & 0.89 & 0.88 & 0.87 & 0.83 & 0.82 & 0.86 & 0.90 \\
\Name{Forest}/\Name{Simple} & 0.94 & 0.51 & 0.36 & 0.30 & 1.02 & 0.80 & 0.61 & 0.41 & 0.89 & 0.70 & 0.59 & 0.54 \\
\hline
\end{tabular}
}\\
\subfloat[Matching time (ms)]{
\label{tab:output:search}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Approach & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Simple} & 525 & 609 & 693 & 1,088 & 469 & 646 & 919 & 1,266 & 448 & 700 & 1,073 & 2,853 \\
\Name{Shared} & 525 & 613 & 719 & 1,148 & 457 & 653 & 923 & 1,304 & 415 & 668 & 1,044 & 2,822 \\
\Name{Forest} & 533 & 596 & 697 & 1,088 & 446 & 626 & 871 & 1,259 & 427 & 663 & 1,027 & 2,796 \\
\hline
\Name{Shared}/\Name{Simple} & 1.00 & 1.01 & 1.04 & 1.06 & 0.98 & 1.01 & 1.00 & 1.03 & 0.92 & 0.95 & 0.97 & 0.99 \\
\Name{Forest}/\Name{Simple} & 1.01 & 0.98 & 1.00 & 1.00 & 0.95 & 0.97 & 0.95 & 0.99 & 0.95 & 0.95 & 0.96 & 0.98 \\
\hline
\end{tabular}
}\\
\subfloat[Average cardinality of $h(s)$]{
\label{tab:output:card}
\begin{tabular}{|l||rrrr|}
\hline
Dataset & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{EnWord} & 1.37 & 2.07 & 3.16 & 4.15 \\
\Name{JaWord} & 1.42 & 1.76 & 2.20 & 3.02 \\
\Name{JaChars} & 1.63 & 2.06 & 2.42 & 2.73 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
Experimental results on memory efficiency in the \Name{Bytewise}, \Name{Charwise}, and \Name{Mapped} schemes.
The memory usage is the total of \Name{BASE}, \Name{CHECK}, \Name{FAIL}, and \Name{OUTPOS} (and the mapping $\pi$ in \Name{Mapped}).
The last rows in Tables (a) and (d) show the different ratios for each result.
}
\label{tab:scheme:stat}
\subfloat[Number of original states ($\times 10^3$)]{
\label{tab:scheme:states}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 2.74 & 25.6 & 237 & 2,129 & 2.96 & 27.9 & 305 & 4,899 & 1.73 & 18.5 & 186 & 1,790 \\
\Name{Charwise} & 2.74 & 25.6 & 237 & 2,124 & 1.43 & 13.0 & 142 & 2,155 & 1.12 & 10.9 & 107 & 1,052 \\
\hline
\Name{Charwise}/\Name{Bytewise} & 1.00 & 1.00 & 1.00 & 1.00 & 0.48 & 0.47 & 0.46 & 0.44 & 0.65 & 0.59 & 0.58 & 0.59 \\
\hline
\end{tabular}
}\\
\subfloat[Proportion of vacant ids (\%)]{
\label{tab:scheme:vacant}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 2.6 & 0.9 & 0.1 & 0.0 & 3.7 & 0.8 & 0.2 & 0.1 & 15.3 & 0.8 & 0.2 & 0.0 \\
\Name{Charwise} & 66.6 & 0.2 & 0.0 & 0.0 & 96.4 & 77.3 & 16.3 & 0.7 & 97.2 & 84.1 & 68.0 & 71.8 \\
\Name{Mapped} & 2.7 & 0.9 & 0.2 & 0.0 & 30.2 & 20.5 & 3.9 & 1.1 & 27.1 & 24.1 & 12.6 & 27.0 \\
\hline
\end{tabular}
}\\
\subfloat[Average number of outgoing transitions for an internal state.]{
\label{tab:scheme:outgoing}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 1.41 & 1.40 & 1.44 & 1.50 & 1.41 & 1.43 & 1.37 & 1.20 & 1.87 & 1.68 & 1.75 & 1.91 \\
\Name{Charwise} & 1.41 & 1.41 & 1.44 & 1.50 & 2.54 & 2.79 & 2.40 & 1.60 & 3.58 & 3.25 & 3.83 & 5.33 \\
\hline
\end{tabular}
}\\
\subfloat[Memory usage (KiB)]{
\label{tab:scheme:memory}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 44 & 404 & 3,712 & 33,276 & 48 & 440 & 4,780 & 76,596 & 32 & 292 & 2,908 & 27,972 \\
\Name{Charwise} & 128 & 401 & 3,707 & 33,193 & 619 & 896 & 2,646 & 33,922 & 619 & 1,067 & 5,240 & 58,318 \\
\Name{Mapped} & 76 & 442 & 3,959 & 33,456 & 187 & 480 & 2,554 & 38,145 & 179 & 384 & 2,144 & 22,778 \\
\hline
\Name{Charwise}/\Name{Bytewise} & 2.91 & 0.99 & 1.00 & 1.00 & 12.89 & 2.04 & 0.55 & 0.44 & 19.34 & 3.65 & 1.80 & 2.08 \\
\Name{Mapped}/\Name{Bytewise} & 1.73 & 1.09 & 1.07 & 1.01 & 3.89 & 1.09 & 0.53 & 0.50 & 5.59 & 1.31 & 0.74 & 0.81 \\
\Name{Mapped}/\Name{Charwise} & 0.59 & 1.10 & 1.07 & 1.01 & 0.30 & 0.54 & 0.97 & 1.12 & 0.29 & 0.36 & 0.41 & 0.39 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
Experimental results on time efficiency in the \Name{Bytewise}, \Name{Charwise}, and \Name{Mapped} schemes.
The last rows in Tables (a) and (c) show the different ratios for each result.
}
\label{tab:scheme}
\subfloat[Number of visiting states during matching ($\times 10^6$)]{
\label{tab:scheme:trans}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 108 & 104 & 107 & 111 & 128 & 128 & 129 & 129 & 129 & 129 & 129 & 131 \\
\Name{Charwise} & 108 & 104 & 107 & 111 & 57 & 61 & 61 & 61 & 59 & 62 & 62 & 62 \\
\hline
\Name{Charwise}/\Name{Bytewise} & 1.00 & 1.00 & 1.00 & 1.00 & 0.44 & 0.48 & 0.47 & 0.47 & 0.45 & 0.48 & 0.48 & 0.48 \\
\hline
\end{tabular}
}\\
\subfloat[Matching time (ms)]{
\label{tab:scheme:search}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 527 & 597 & 689 & 1,057 & 454 & 644 & 896 & 1,254 & 406 & 648 & 1,021 & 2,735 \\
\Name{Charwise} & 550 & 628 & 720 & 1,098 & 362 & 444 & 563 & 809 & 356 & 507 & 661 & 1,812 \\
\Name{Mapped} & 576 & 665 & 748 & 1,157 & 310 & 402 & 484 & 731 & 304 & 439 & 620 & 1,403 \\
\hline
\Name{Charwise}/\Name{Bytewise} & 1.04 & 1.05 & 1.04 & 1.04 & 0.80 & 0.69 & 0.63 & 0.65 & 0.88 & 0.78 & 0.65 & 0.66 \\
\Name{Mapped}/\Name{Bytewise} & 1.09 & 1.11 & 1.09 & 1.09 & 0.68 & 0.62 & 0.54 & 0.58 & 0.75 & 0.68 & 0.61 & 0.51 \\
\Name{Mapped}/\Name{Charwise} & 1.05 & 1.06 & 1.04 & 1.05 & 0.86 & 0.91 & 0.86 & 0.90 & 0.85 & 0.87 & 0.94 & 0.77 \\
\hline
\end{tabular}
}\\
\subfloat[Construction time (ms)]{
\label{tab:scheme:build}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Scheme & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Bytewise} & 0.12 & 1.34 & 21 & 244 & 0.13 & 1.44 & 27 & 387 & 0.09 & 1.2 & 20 & 275 \\
\Name{Charwise} & 0.14 & 0.79 & 18 & 199 & 0.32 & 1.09 & 163 & 1,829 & 0.29 & 2.3 & 134 & 21,184 \\
\Name{Mapped} & 0.09 & 0.81 & 18 & 204 & 0.06 & 1.50 & 102 & 1,251 & 0.08 & 1.4 & 45 & 9,107 \\
\hline
\Name{Charwise}/\Name{Bytewise} & 1.18 & 0.59 & 0.86 & 0.81 & 2.51 & 0.76 & 6.03 & 4.72 & 3.14 & 1.92 & 6.72 & 77.1 \\
\Name{Mapped}/\Name{Bytewise} & 0.80 & 0.60 & 0.86 & 0.83 & 0.44 & 1.04 & 3.77 & 3.23 & 0.83 & 1.22 & 2.25 & 33.1 \\
\Name{Mapped}/\Name{Charwise} & 0.68 & 1.03 & 1.01 & 1.03 & 0.17 & 1.37 & 0.62 & 0.68 & 0.26 & 0.64 & 0.33 & 0.43 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
\R{Experimental results on memory efficiency, matching time, and CPU instructions when varying the memory layout of the $\pi$ data structure in the \Name{Mapped} scheme.
\Name{4B} and \Name{3B} indicate the cases that $\pi$ is implemented with four- and three-byte arrays, respectively.
The memory usage is the total of \Name{BASE}, \Name{CHECK}, \Name{FAIL}, \Name{OUTPOS}, and $\pi$.
The last rows in each table show the different ratios for each result.}
}
\label{tab:scheme:3B}
\subfloat[Memory usage (KiB)]{
\label{tab:scheme:3B:memory}
\begin{tabular}{|l||rrrr|rrrr|}
\hline
  & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Layout & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{4B} & 187 & 480 & 2,554 & 38,145 & 179 & 384 & 2,144 & 22,778 \\
\Name{3B} & 148 & 424 & 2,492 & 37,121 & 140 & 344 & 2,088 & 22,716 \\
\hline
\Name{3B}/\Name{4B} & 0.79 & 0.88 & 0.98 & 0.97 & 0.78 & 0.90 & 0.97 & 1.00 \\
\hline
\end{tabular}
}\\
\subfloat[Matching time (ms)]{
\label{tab:scheme:3B:match}
\begin{tabular}{|l||rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Layout & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{4B} & 310 & 402 & 484 & 731 & 304 & 439 & 620 & 1,403 \\
\Name{3B} & 334 & 430 & 526 & 783 & 320 & 451 & 618 & 1,456 \\
\hline
\Name{3B}/\Name{4B} & 1.08 & 1.07 & 1.09 & 1.07 & 1.06 & 1.03 & 1.00 & 1.04 \\
\hline
\end{tabular}
}\\
\subfloat[CPU instructions ($10^6$)]{
\label{tab:scheme:3B:instructions}
\begin{tabular}{|l||rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Layout & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{4B} & 4,185 & 4,446 & 4,605 & 4,769 & 4,299 & 4,609 & 4,812 & 4,953 \\
\Name{3B} & 4,517 & 4,798 & 4,948 & 5,100 & 4,635 & 4,949 & 5,138 & 5,267 \\
\hline
\Name{3B}/\Name{4B} & 1.08 & 1.08 & 1.07 & 1.07 & 1.08 & 1.07 & 1.07 & 1.06 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
\R{Proportion of the number of L3-load misses over that of L1 loads when the number of patterns is $10^6$.}
}
\label{tab:layout:ratio}
\begin{tabular}{|l||rrr|}
\hline
Layout & \Name{EnWord} & \Name{JaWord} & \Name{JaChars} \\
\hline\hline
\Name{Individual} & 0.7\% & 1.0\% & 7.3\% \\
\Name{Packed} & 0.3\% & 0.4\% & 3.2\% \\
\hline
\end{tabular}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
Experimental results for the \Name{Basic} and \Name{Compact} formats.
The memory usage is the total of \Name{BASE}, \Name{CHECK}, \Name{FAIL}, and \Name{OUTPOS}.
The last row in each table shows the different ratios for each result.
}
\label{tab:format}
\subfloat[Memory usage (KiB)]{
\label{tab:format:memory}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Format & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Basic} & 44.0 & 404 & 3,712 & 33,276 & 48.0 & 440 & 4,780 & 76,544 & 32.0 & 292 & 2,908 & 27,972 \\
\Name{Compact} & 33.0 & 303 & 2,784 & 24,957 & 36.0 & 330 & 3,585 & 57,408 & 24.0 & 219 & 2,181 & 20,979 \\
\hline
\Name{Compact}/\Name{Basic} & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 & 0.75 \\
\hline
\end{tabular}
}\\
\subfloat[Matching time (ms)]{
\label{tab:format:match}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Format & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Basic} & 523 & 600 & 696 & 1,082 & 447 & 632 & 879 & 1,234 & 406 & 651 & 1,038 & 2,733 \\
\Name{Compact} & 545 & 606 & 712 & 1,052 & 473 & 633 & 893 & 1,226 & 415 & 609 & 1,028 & 2,439 \\
\hline
\Name{Compact}/\Name{Basic} & 1.04 & 1.01 & 1.02 & 0.97 & 1.06 & 1.00 & 1.02 & 0.99 & 1.02 & 0.94 & 0.99 & 0.89 \\
\hline
\end{tabular}
}\\
\subfloat[Construction time (ms)]{
\label{tab:format:build}
\begin{tabular}{|l||rrrr|rrrr|rrrr|}
\hline
 & \multicolumn{4}{c|}{\Name{EnWord}} & \multicolumn{4}{c|}{\Name{JaWord}} & \multicolumn{4}{c|}{\Name{JaChars}} \\
Format & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M & 1K & 10K & 100K & 1M \\
\hline\hline
\Name{Basic} & 0.11 & 1.06 & 19.2 & 207 & 0.13 & 1.19 & 22.4 & 331 & 0.08 & 0.81 & 14.8 & 200 \\
\Name{Compact} & 0.14 & 1.30 & 23.5 & 249 & 0.14 & 1.39 & 32.7 & 182,015 & 0.09 & 0.91 & 16.0 & 226 \\
\hline
\Name{Compact}/\Name{Basic} & 1.25 & 1.23 & 1.22 & 1.20 & 1.09 & 1.17 & 1.46 & 549 & 1.09 & 1.12 & 1.08 & 1.13 \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
The average number of verifications per vacant search when using \Name{Chain}.
The number of patterns in each dictionary is one million.
}
\label{tab:constr:verif}
\begin{tabular}{|l||rrr|}
\hline
Method & \Name{EnWord} & \Name{JaWord} & \Name{JaChars} \\
\hline\hline
\Name{Bytewise} + \Name{Basic} & 2.8 & 2.8 & 6.6 \\
\Name{Bytewise} + \Name{Compact} & 4.6 & 5383.3 & 7.4 \\
\Name{Mapped} & 2.5 & 84.4 & 4934.5 \\
\hline
\end{tabular}
\end{table}

\begin{table}[p]
\footnotesize
\centering
\caption{
The number of L3-load misses occurring during a pattern matching with different traversal orders ({$\times 10^3$}).
The number of patterns is fixed to $10^6$.
The last row shows the different ratios for each result.
}
\label{tab:order:cache}
\begin{tabular}{|l||rr|rr|rr|}
\hline
 & \multicolumn{2}{c|}{\Name{EnWord}} & \multicolumn{2}{c|}{\Name{JaWord}} & \multicolumn{2}{c|}{\Name{JaChars}} \\
Order & \Name{Bytewise} & \Name{Mapped} & \Name{Bytewise} & \Name{Mapped} & \Name{Bytewise} & \Name{Mapped} \\
\hline\hline
\Name{LexBFS} & 2,485 & 2,967 & 4,301 & 3,157 & 31,999 & 17,719 \\
\Name{LexDFS} & 2,303 & 2,888 & 3,209 & 2,944 & 28,804 & 17,917 \\
\hline
\Name{LexDFS}/\Name{LexBFS} & 0.93 & 0.97 & 0.75 & 0.93 & 0.90 & 1.01 \\
\hline
\end{tabular}
\end{table}

